LiLo-VLA: Compositional Long-Horizon Manipulation via Linked Object-Centric Policies

General-purpose robots must master long-horizon manipulation, defined as tasks involving multiple kinematic structure changes (e.g., attaching or detaching objects) in unstructured environments. While Vision-Language-Action (VLA) models offer the potential to master diverse atomic skills, they struggle with the combinatorial complexity of sequencing them and are prone to cascading failures due to environmental sensitivity. To address these challenges, we propose LiLo-VLA (Linked Local VLA), a modular framework capable of zero-shot generalization to novel long-horizon tasks without ever being trained on them. Our approach decouples transport from interaction: a Reaching Module handles global motion, while an Interaction Module employs an object-centric VLA to process isolated objects of interest, ensuring robustness against irrelevant visual features and invariance to spatial configurations. Crucially, this modularity facilitates robust failure recovery through dynamic replanning and skill reuse, effectively mitigating the cascading errors common in end-to-end approaches. We introduce a 21-task simulation benchmark consisting of two challenging suites: LIBERO-Long++ and Ultra-Long. In these simulations, LiLo-VLA achieves a 69% average success rate, outperforming Pi0.5 by 41% and OpenVLA-OFT by 67%. Furthermore, real-world evaluations across 8 long-horizon tasks demonstrate an average success rate of 85%. Project page: https://yy-gx.github.io/LiLo-VLA/.

==> tables/fig_perf_oss.tex <==
% --- Ensure these are in your preamble ---
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.18}
% \usetikzlibrary{patterns} 

\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=14pt,
            width=0.48\textwidth,
            height=6.0cm,
            ymin=0.2, ymax=1.35,    % Y-axis range adjusted for space
            ylabel={\textbf{Success Rate}},
            xtick={1,2,3},
            xticklabels={3rd Person, Both Views, \textbf{Wrist Only}},
            xticklabel style={font=\small, align=center, yshift=-4pt},
            ytick={0.2, 0.4, 0.6, 0.8, 1.0},
            % Value Labels (Numbers on bars) settings
            nodes near coords,
            every node near coords/.append style={
                font=\tiny,         % Smaller font to prevent overlap
                /pgf/number format/fixed, 
                /pgf/number format/precision=2, 
                yshift=3pt          % Lift numbers up away from the bar
            },
            % Legend settings
            legend style={
                at={(0.02,0.98)}, 
                anchor=north west, 
                font=\scriptsize, 
                columns=1,
                legend image post style={scale=0.8} % Scale down legend icons
            },
            ymajorgrids=true,
            grid style={dashed, gray!20},
            enlarge x limits=0.25,
        ]

        % ======================================================
        % MANUAL LEGEND (Neutral Colors)
        % ======================================================
        % 1. Neutral Gray Solid Box -> Original Task
        \addlegendimage{ybar, fill=gray, draw=none, bar width=10pt}
        \addlegendentry{Original Task}
        
        % 2. Neutral Gray Hatched Box -> Under OSS Shift
        \addlegendimage{ybar, fill=white, pattern=north east lines, pattern color=gray, draw=gray, bar width=10pt}
        \addlegendentry{Under OSS Shift}


        % ======================================================
        % DATA PLOTS (Distinct Colors)
        % Using 'forget plot' so they don't mess up the manual legend
        % ======================================================

        % --- GROUP 1: 3rd Person (Teal) ---
        % Original
        \addplot[fill=teal!60, draw=none, bar shift=-7pt, forget plot] 
            coordinates {(1, 0.57)};
        % OSS
        \addplot[pattern=north east lines, pattern color=teal!60, draw=teal!60, bar shift=7pt, forget plot] 
            coordinates {(1, 0.40)};

        % --- GROUP 2: Both Views (SlateBlue/Purple-ish) ---
        % Original
        \addplot[fill=blue!50!violet, draw=none, bar shift=-7pt, forget plot] 
            coordinates {(2, 0.80)};
        % OSS
        \addplot[pattern=north east lines, pattern color=blue!50!violet, draw=blue!50!violet, bar shift=7pt, forget plot] 
            coordinates {(2, 0.65)};

        % --- GROUP 3: Wrist Only (Orange - Hero Color) ---
        % Original
        \addplot[fill=orange, draw=none, bar shift=-7pt, forget plot] 
            coordinates {(3, 0.88)};
        % OSS
        \addplot[pattern=north east lines, pattern color=orange, draw=orange, bar shift=7pt, forget plot] 
            coordinates {(3, 0.74)};


        % ======================================================
        % RPD ANNOTATIONS (Placed High)
        % ======================================================
        % Placed centrally above each group, slightly higher than the max bar
        
        % 3rd Person Drop
        \node[font=\bfseries\tiny, text=teal!60] at (axis cs:1, 0.70) {$\downarrow$29.8\%};
        
        % Both Views Drop
        \node[font=\bfseries\tiny, text=blue!50!violet] at (axis cs:2, 0.90) {$\downarrow$18.8\%};
        
        % Wrist Only Drop
        \node[font=\bfseries\tiny, text=orange] at (axis cs:3, 1.05) {$\downarrow$15.9\%};
        
        \end{axis}
    \end{tikzpicture}
    \caption{\textbf{Visual Robustness Comparison.} Evaluation of policy robustness under Observation Space Shift (OSS). Solid bars denote original performance; hatched bars denote performance under shift. While 3rd-person (Teal) and Multi-view (Purple) policies degrade significantly, the \textcolor{orange}{\textbf{Wrist-Only}} policy (Ours, Orange) demonstrates superior robustness with the lowest relative performance drop (RPD).}
    \label{fig:ablation_vision}
\end{figure}
